OrgMining 2.0: A Novel Framework for Organizational Model Mining from Event Logs

Providing appropriate structures around human resources can streamline operations and thus facilitate the competitiveness of an organization. To achieve this goal, modern organizations need to acquire an accurate and timely understanding of human resource grouping while faced with an ever-changing environment. The use of process mining offers a promising way to help address the need through utilizing event log data stored in information systems. By extracting knowledge about the actual behavior of resources participating in business processes from event logs, organizational models can be constructed, which facilitate the analysis of the de facto grouping of human resources relevant to process execution. Nevertheless, open research gaps remain to be addressed when applying the state-of-the-art process mining to analyze resource grouping. For one, the discovery of organizational models has only limited connections with the context of process execution. For another, a rigorous solution that evaluates organizational models against event log data is yet to be proposed. In this paper, we aim to tackle these research challenges by developing a novel framework built upon a richer definition of organizational models coupling resource grouping with process execution knowledge. By introducing notions of conformance checking for organizational models, the framework allows effective evaluation of organizational models, and therefore provides a foundation for analyzing and improving resource grouping based on event logs. We demonstrate the feasibility of this framework by proposing an approach underpinned by the framework for organizational model discovery, and also conduct experiments on real-life event logs to discover and evaluate organizational models.

==> sections/archived/1_intro_v1.tex <==
\section{Introduction} \label{sec:intro}
Information systems such as Enterprise Resource Planning systems and Workflow Management systems provide solid infrastructural support for modern organizations to effectively manage their end-to-end business processes. The deployment and operation of such Process-Aware Information Systems result in a considerable amount of process-related data being generated and stored. These data record the actual execution of business processes. Advances in process mining research in the recent decades offer an ever-expanding set of methods and tools which enable process owners and business analysts to extract knowledge from these data readily available in many organizations~\cite{vanderaalst2016process}, often in the form of event logs. Insights gained from using process mining may subsequently contribute to diagnosing existing performance issues or improving the design of a process. 

Effective process management requires various aspects of a process to be taken into account, and process mining research thereby adopts a multiple perspective view on process-related data. The organizational perspective considers the human resources involved in a business process, mainly those acting as participating workers in process execution. The fact that human resource behavior impacts the execution and thus the performance of business processes has been recognized by the literature~\cite{nakatumba2013resource,song2008towards,pika2017mining,huang2012resource,suriadi2017discovering}.
In the context of business process management, human resources are often referred to in the form of resource classes~\cite{dumas2018fundamentals}, in the sense that resources with the same group identity could be considered interchangeable in terms of carrying out certain types of work in a process. 
For instance, a common approach of distributing work items in process execution is based on business roles assigned to individual resources, with the expectation that those having the same role could work on it~\cite{russell2016}. 
Besides business roles, various kinds of resource grouping mechanisms exist in an organization, e.g., roles, departments, cross-functional teams, which contribute an important factor in managing the human resource aspect of a business process. The need for understanding and (re)designing resource grouping should be adequately addressed such that it aligns with the overall strategies for overseeing processes, as evidenced by the organizational structure-related best practices for business process redesign~\cite{reijers2005best}. In a broader context, appropriate structural decisions of human resources would also benefit the performance of an organization~\cite{daft2010organization}.

%Process mining research devoted to the organizational perspective of processes is known as organizational mining~\cite{song2008towards}, in which the topic of \emph{organizational model mining} addresses the study of resource grouping in the context of business processes.
In process mining research, the topic of \emph{organizational model mining}~\cite{song2008towards} addresses the study of resource grouping in the context of business processes.
The aim is to find groups of resources having similar characteristics in process execution using event logs, and with that a number of methods were proposed in literature to discover different forms of ``organizational models'' depending on the contexts. An example of such methods targets the discovery of business roles of resources from event logs based on cluster analysis~\cite{jin2007organizational}.

Nevertheless, the state-of-the-art work on organizational model mining focuses only on recovering the underlying, existing structural patterns of resource groups in an organization as reflected by process execution, i.e., how resources may be linked with one another as groups. Meanwhile, the behavioral patterns of resource groups, i.e., how groups of resources perform in process execution, still remain an issue to be further explored. This incurs the currently missing link between derived organizational models and business process underlying the event log data, and subsequently poses a challenge of further utilizing the extracted information to improve resource grouping. 
It should also be noted that existing work on the topic adopted context- or technique-specific solutions for evaluating discovered organizational models, e.g., referring to prior knowledge about the organizational structure~\cite{song2008towards}, or assessing the quality of the produced resource grouping as clusters~\cite{jin2007organizational}, while lacks in a general and rigorous way of evaluating organizational models against the source process-related data (as the conformance checking for process model discovery~\cite{rozinat2008,adriansyah2013,Garcia-Banuelos2018}). This implies yet another gap that may hinder process mining research from applying to the study of resource grouping in business process context. 


In this paper, we report our contribution which addresses the aforementioned research gaps. 
We present a novel framework built upon a richer definition of organizational models linking resources and resource groups with business processes, thus enabling more in-depth resource-centric analysis coupled with process context.
Through introducing the notions and measures for model conformance, this framework allows the evaluation of an organizational model with reference to event log data, without being bound by how the model may be constructed. 
As an example, we demonstrate an approach under the framework for discovering organizational models from a given event log. 
Furthermore, a series of experiments were conducted on real-life event log data, which showcased the feasibility of the proposed framework and approach in terms of both the discovery and conformance checking of organizational models.
Open-source software was developed as artifacts that implement the proposals in the paper.
We expect that the establishment of such a framework will empower the use of process mining to analyze and improve resource grouping in business processes, while also unleashes the possibilities for future research with regard to mining the organizational perspective. 

The remainder of the paper is structured as follows. 
Section~\ref{sec:related} details the introduction to the state-of-the-art work of process mining research on the organizational perspective, with a specific focus on the topic of organizational model mining.
Section~\ref{sec:framework} elaborates on the novel framework proposed in this paper. 
Subsequently, Section~\ref{sec:approach} presents an approach that realizes the discovery of organizational models discussed in the framework.
Section~\ref{sec:implementation} provides the information about the related software implementation of our work.
Section~\ref{sec:evaluation} reports the evaluation of our work through experiments and discusses the findings.
Finally, Section~\ref{sec:conclusion} concludes the paper with a summary and the outlook for a range of future research topics that could be built upon the current work.




==> sections/archived/1_intro_v2.tex <==
\section{Introduction} \label{sec:intro}
% Organization: people, processes and changes
%Modern organizations are comprised of people deliberately structured in different forms of groups and strive to attain desired goals~\cite{daft2010organization}. 
Modern organizations are comprised of people structured in different forms of groups, and work by employees within an organization is often directed by end-to-end business processes towards delivering valued outcomes achieving the organization's goals~\cite{daft2010organization}. 
Faced with a rapidly changing environment, organizations today are required to constantly adapt and respond to various demands in order to keep being competitive. Having flexible and proper structural settings for human resources would facilitate addressing such a challenge, as evidenced by the organizational structure-related practices for business process redesign~\cite{reijers2005best}. For this purpose, managers in an organization need to both obtain and maintain an accurate and timely understanding of human resource grouping alongside evolving processes, and thus inform appropriate decisions. %about resource grouping. 
This, however, could hardly be sufficed by merely having a static ``as-is'' organizational chart.

% Information Systems, data and process mining
A possible way to address the above need %of supporting such inquiries 
is through utilizing data related to process execution readily available in many information systems, such as enterprise resource planning \textsc{(erp)} systems, deployed in today's organizations~\cite{vanderaalst2016process}. These data, often stored as event logs, could contain information recording %the actual situation of 
how human resources {\it actually} carried out work when participating in processes. 
Advances in process mining research offer an ever-expanding set of methods to dive into event logs and extract knowledge about historical behavior of a process and its participants and therefore support decision-making. Further actions could impact process execution and produce new event log data, which may then trigger a next round of analysis and inform subsequent decisions. 
In this sense, process mining may be applied to support management by enabling the cycle of continuously monitoring as well as improving structural settings of human resources, and thus contribute to the competitiveness of an organization.

% Process mining for the purpose: organizational model mining
In process mining research, studies focused on human resource grouping are known as the topic of organizational model mining. State-of-the-art work aims at finding groups of human resources having similar characteristics in process execution, e.g., mining business roles of resources using event logs~\cite{jin2007organizational}. 
% State-of-the-art organizational model mining: what are the gaps
Nevertheless, certain gaps exist which hinder the current research from being applied to tackle the aforementioned challenge. 
For one, existing research focuses only on recovering the underlying, existing structural patterns of resource groups in an organization as reflected by historical process execution (i.e., how resources may be linked with one another as groups), without further exploring the behavioral patterns of resource groups (i.e., what and how resource groups perform in process execution). Consequently, it remains unclear how to interpret the derived results; also, such a missing link between resource groups and processes may prevent one from gaining insights on further revisions through incorporating process knowledge.
%subsequently poses a challenge of further utilizing the extracted information to improve resource grouping.
For another, it should be noted that the existing work fails to devise a general and rigorous way of evaluating organizational models against event logs, and is limited to merely assessing the discovery results using context- or technique-specific solutions. Examples include referring to prior knowledge about the ``official'' organizational structure~\cite{song2008towards}; or assessing the quality of the produced resource grouping as clusters~\cite{jin2007organizational} due to the use of cluster analysis technique. Such a lack leaves the conducted evaluations ill-posed: context-specific prior knowledge could indeed be different from the \textit{de facto} behavior recorded in event logs as organizational structure may have evolved while processes do; and technique-specific evaluate could be biased as it depends on the nature of specific technique adopted.
Comparing organizational models with event logs as the reference is needed for effective evaluation of any mining result and thus ensuring the value of subsequent analysis based on it.

% Contributions claimed in this paper
In this paper, we report our contribution which addresses these research gaps. 
We present a novel framework built upon a richer definition of organizational models linking resources and resource groups with business processes, thus enabling more in-depth resource-centric analysis coupled with process context.
Through introducing the notions and measures for model conformance, this framework allows the evaluation of an organizational model with reference to event log data, without being bound by how the model may be constructed. 
As an example, we demonstrate an approach under the framework for discovering organizational models from a given event log. 
Furthermore, a series of experiments were conducted on real-life event log data, which showcased the feasibility of the proposed framework and approach in terms of both the discovery and conformance checking of organizational models.
Open-source software was developed as artifacts that implement the proposals in the paper.
We expect that the establishment of such a framework will empower the use of process mining to support analyzing and improving resource grouping for organizational management, while also unleashes the possibilities for future process mining research with regard to the organizational perspective. 

% Roadmap for the paper
The remainder of the paper is structured as follows. 
Section~\ref{sec:related} details the introduction to the state-of-the-art work of process mining research on the organizational perspective, with a specific focus on the topic of organizational model mining.
Section~\ref{sec:framework} elaborates on the novel framework proposed in this paper. 
Subsequently, Section~\ref{sec:approach} presents an approach that realizes the discovery of organizational models discussed in the framework.
Section~\ref{sec:implementation} provides the information about the related software implementation of our work.
Section~\ref{sec:evaluation} reports the evaluation of our work through experiments and discusses the findings.
Finally, Section~\ref{sec:conclusion} concludes the paper with a summary and the outlook for a range of future research topics that could be built upon the current work.




==> sections/archived/2_related_v1.tex <==
\section{Related Work} 
\label{sec:related}

%\section{Background and Related Work} 
% more precisely, this section discusses background and related work. 
% we may also categorise the related work in a way similar to Schonig et al.'s paper

% ----- Temporarily cut out to keep intro and related work in the first page ----- %
% Background: (include necessary background information about BPM for TKDE audience) knowledge about business process, multiple perspectives of processes, resource/organizational perspective, process data, event logs, process mining, organizational mining, organizational model mining

% 1. Overview of organizational mining
\subsection{Organizational Mining}
Process mining research that aims at extracting human-resource-related insights from event log data is also known as organizational mining. Research on organizational mining can be dated back to the early work by van der Aalst and Song et al.~\cite{vanderaalst2004mining,vanderaalst2005discovering}, which enables extracting inter-resource relationships from event logs to build a resource social network, allowing subsequent social network analysis to be applied to uncover potential communication patterns among resources or to distinguish different groups of resources, etc.
%
Ly et al.~\cite{ly2005mining} proposed the concept of staff assignment rules mining which focuses on extracting inherent rules that decide the assignment of tasks to resources in process execution. These mark a starting point of process mining research devoted to the resource perspective of business process execution. 
% other than control-flow, case, etc. 
%
Subsequent work on organizational mining extends the above research topics of resource social network mining (e.g.,~\cite{liu2013accelerating}) and rule mining (e.g.,~\cite{rinderlema2007,schonig2016a}), as well as introduces the topics of organizational model mining (e.g.,~\cite{jin2007organizational,burattin2013business,song2008towards,appice2018towards,yang2018finding}) and resource behavioral profile mining (e.g., \cite{nakatumba2009analyzing,pika2017mining,huang2012resource,suriadi2017discovering}).

A conceptual framework for organizational mining proposed by Song and van der Aalst~\cite{song2008towards} articulates three research themes for organizational mining, in line with the general idea of process mining research. The framework can be used for positioning existing studies and guiding prospective work on organizational mining: 
\textit{Discovery} refers to deriving models to describe the reality as reflected by event logs.
\textit{Conformance checking} refers to investigating the alignment between modeled behavior and actual behavior recorded in event logs. An existing model and a related event log are both given as inputs and the possible deviation between the model and reality can be investigated, and the results may help address concerns including diagnosing problematic models and evaluating model discovery results.
\textit{Extension}, or more generally, \textit{enhancement}, refers to enriching and/or improving existing models using knowledge extracted from event logs based on discovery and/or conformance checking. The inputs include an ``as-is'' model and an event log, and a model added with information extracted from the log, or a model changed for improvement, is produced.

The focus of this paper is to utilize process mining to support the analysis and improvement of resource grouping based on event log data, which aligns with the topic of organizational model mining that concerns deriving knowledge about organizational structures~\cite{song2008towards}. To this end, we will investigate the state-of-the-art research on organizational model mining by adopting the conceptual framework by Song and van der Aalst~\cite{song2008towards} as a reference.

\subsection{Organizational Model Mining}
Existing work on organizational model mining employs different views towards the definition of an organizational model. In the literature, an organizational model may be viewed as
(1) a set of business roles~\cite{jin2007organizational,baumgrass2011deriving,zhao2012mining,burattin2013business,ye2018mining} which correspond to different expertise or designated permissions of resources, 
(2) a set of resource groups of which the meaning depends on the context~\cite{song2008towards,ni2011mining,appice2018towards,yang2018finding} such as units, project teams, departments, etc., or
(3) a communication structure depicted as a graph where nodes are resources and links represent the coordination among resources annotated by specific semantics~\cite{li2011a,hanachi2012performative,sellami2012an,bouzguenda2015an} such as subordination, cooperation, etc.

The discovery of organizational models from event logs is usually approached by aggregating similar resources based on how they performed in process execution, which is done by using either cluster analysis or social network analysis (i.e., finding connected components or community structures in a constructed resource network). An important component shared by existing approaches for organizational model discovery is to describe resource characteristics in terms of  % process execution. 
%The state-of-the-art research mainly considers 
(1) how resources originated different tasks~\cite{jin2007organizational,baumgrass2011deriving,zhao2012mining,ye2018mining,song2008towards,ni2011mining,appice2018towards,yang2018finding}, or 
(2) resource interactions~\cite{burattin2013business,li2011a,hanachi2012performative,sellami2012an,bouzguenda2015an}, in process execution, e.g., handovers between the execution of subsequent tasks or delegations between superior and subordinate resources. 
%From the viewpoint of different perspectives of business processes, the above strategies for characterizing resource behavior in process execution focus only on the control-flow aspect. 
However, the above strategies for characterizing resource behavior focus only on the task or activity aspect of process execution. Event logs often record information about other aspects, such as %various types of information information relevant to 
business cases or time patterns, of process execution. Incorporating information on multiple aspects of process execution contributes to a better understanding and planning of the deployment of human resources~\cite{pika2017mining}, 
%as evidenced by research on mining resource behavioral profiles
yet this still remains an open issue in the current organizational model mining research.

With regard to the evaluation of discovery results (if conducted), there are two typical solutions in the existing studies. 
%For one, the evaluation was done depending on the 
One solution approaches it by assessing the effectiveness of the techniques adopted for model discovery, e.g., evaluating the quality of the derived clusters~\cite{jin2007organizational} or detected communities~\cite{ye2018mining,appice2018towards}. 
However, such evaluation is technique-specific and may be biased as the method and criteria are often dependent upon the selected techniques. 
The other solution compares the discovery results with existing domain knowledge, %used as a reference, 
e.g., official organizational structure~\cite{burattin2013business,song2008towards,yang2018finding,li2011a}. 
%Yet none of the studies to date concerns the evaluation by comparing the derived models with the source event log data, which may raise questions around the validity of the evaluation results. %On the other hand, 
However, the reality (as reflected by event log data) may have deviated from the domain knowledge, %obtained in the first place, 
which makes it less plausible to use context knowledge as a reference for evaluating models discovered from event logs.

%The above gap in terms of evaluation is also reflected by the limited amount of literature that directly concerns the issue of conformance checking on organizational models. 
So far, there is only a limited amount of literature addressing the above issues of conformance checking on organizational models. 
Baumgrass et al.~\cite{baumgrass2012conformance} proposed an approach that checks if process execution recorded in an event log conforms to given Role-Based Access Control (RBAC) policies, following their previous work~\cite{baumgrass2011deriving} on deriving RBAC models from event logs. The given set of RBAC policies, i.e., the organizational model in the view of the authors, is translated to Linear Temporary Logic (LTL) statements and used to compare with the event log to reveal violations of these policies in reality. To our knowledge, this is the only existing work that is in line with the idea of conformance checking for organizational models.
The lack of research attention for conformance checking from the organizational perspective of business processes is also evidenced by a literature review on the topic of conformance checking~\cite{Dunzer2019}.



In addition, some existing research addressed multi-perspective conformance checking in the broader field of process mining, which indirectly considers the organizational perspective~\cite{deleoni2012data,taghiabadi2014compliance,mannhardt2016balanced}. Measures including fitness~\cite{deleoni2012data} and precision~\cite{mannhardt2016balanced} were proposed to quantify the extent of alignment (or misalignment) between a process model and an event log, taking into account situations where, e.g., a resource executed some tasks without having the qualified role. Other studies focused on the extension (enhancement) of organizational models. Examples include enriching a set of resource groups with the interaction information~\cite{song2008towards} to help reveal patterns of communication among groups; and utilizing time information to track the changes of organizational models over a certain period of time~\cite{appice2018towards} or to conduct real-time analysis~\cite{vanzelst2016online}.
%There exists certain research that addresses 

The review of organizational model mining literature shows that the majority %proportion 
of the state-of-the-art research has been devoted to model discovery. Nevertheless, certain research issues remain open, including the underused event log information related to multiple aspects of processes when conducting the discovery of organizational models, and a proper solution for evaluating the discovered models. Moreover, the topics of conformance checking and enhancement of organizational models are yet to be further explored. From a process mining point of view, developing comprehensive methods for conformance checking and enhancement of organizational models may facilitate  %supporting 
appropriate and timely revision or improvement of human resource grouping, based on analyzing existing group settings and event log data simultaneously.


